Regularizing Self-supervised 3D Scene Flows with Surface Awareness and Cyclic Consistency

Learning without supervision how to predict 3D scene flows from point clouds is essential to many perception systems. We propose a novel learning framework for this task which improves the necessary regularization. Relying on the assumption that scene elements are mostly rigid, current smoothness losses are built on the definition of "rigid clusters" in the input point clouds. The definition of these clusters is challenging and has a significant impact on the quality of predicted flows. We introduce two new consistency losses that enlarge clusters while preventing them from spreading over distinct objects. In particular, we enforce \emph{temporal} consistency with a forward-backward cyclic loss and \emph{spatial} consistency by considering surface orientation similarity in addition to spatial proximity. The proposed losses are model-independent and can thus be used in a plug-and-play fashion to significantly improve the performance of existing models, as demonstrated on two most widely used architectures. We also showcase the effectiveness and generalization capability of our framework on four standard sensor-unique driving datasets, achieving state-of-the-art performance in 3D scene flow estimation. Our codes are available on https://github.com/ctu-vras/sac-flow.

==> consider.tex <==
\section{to consider}

\subsection{Commands and Packages That May Not Be Used}
\begin{table*}[t]
\centering

\begin{tabular}{l|l|l|l}
\textbackslash abovecaption &
\textbackslash abovedisplay &
\textbackslash addevensidemargin &
\textbackslash addsidemargin \\
\textbackslash addtolength &
\textbackslash baselinestretch &
\textbackslash belowcaption &
\textbackslash belowdisplay \\
\textbackslash break &
\textbackslash clearpage &
\textbackslash clip &
\textbackslash columnsep \\
\textbackslash float &
\textbackslash input &
\textbackslash input &
\textbackslash linespread \\
\textbackslash newpage &
\textbackslash pagebreak &
\textbackslash renewcommand &
\textbackslash setlength \\
\textbackslash text height &
\textbackslash tiny &
\textbackslash top margin &
\textbackslash trim \\
\textbackslash vskip\{- &
\textbackslash vspace\{- \\
\end{tabular}
%}
\caption{Commands that must not be used}
\label{table1}
\end{table*}

\begin{table}[t]
\centering
%\resizebox{.95\columnwidth}{!}{
\begin{tabular}{l|l|l|l}
    authblk & babel & cjk & dvips \\
    epsf & epsfig & euler & float \\
    fullpage & geometry & graphics & hyperref \\
    layout & linespread & lmodern & maltepaper \\
    navigator & pdfcomment & pgfplots & psfig \\
    pstricks & t1enc & titlesec & tocbind \\
    ulem
\end{tabular}
\caption{LaTeX style packages that must not be used.}
\label{table2}
\end{table}

==> equations.tex <==
\subsection{Notation}
\begin{itemize}
    \item Point clouds $P$ and $Q$ and Euclidian Nearest Neighborhood NN
    \item $i$ index of point from point cloud $P$, $\tau$ is time of frame
    \item $\omega$ parameters of the network producing $\theta$ and $t_i$
    \item $\theta_i$ rotation per point
    \item $t_i$ translation per point
    \item $C$ rigid cluster from instance segmentation
    \item $o_i^c$ instance mask probabilities of cluster
    \item $b_c$ box parameters per cluster
    \item $x_c$ center of the box (or cluster)
    \item $U$ box coverage function
\end{itemize}

\subsection{Losses}

\subsubsection{Rigid movement with parameterized movement and instance probability.}

\begin{equation}
    \mathcal{L}_{rigid} = \sum_{i\in P} \sum_{c \in C} o_i^c \| R(\theta_i) (p_i - x_c) + t_i - NN(p_i, Q) \|
\end{equation}

\subsubsection{Smoothness regularizer.}
Every point from cluster will have the same parameters for rigid transformation, for one cluster:
% can be written together with L_rigid

\begin{equation}
    \mathcal{L}_{smooth} = \sum_{i,j \in c} \| t_i - t_j \| + \| \theta_i - \theta_j \| + \| \theta_i \|    
\end{equation}

Last part of the equation is allowing only small changes in rotation

\subsubsection{Cyclic Smoothness regularizer.}
cyclic smoothness propagate instance probabilities and rigid parameters in clusters discovered by flow.

\begin{equation}
    \mathcal{L}_{cyclic} = - \sum_{c \in C} \| o_i^c \| + \sum_{\tau \in T} \| \theta_i^{\tau} - \theta_i^{\tau+1} \| + \sum_{\tau \in T} \| t_i^{\tau} - t_i^{\tau+1} \| + 
\end{equation}

\subsubsection{Shape loss.}
Aproximating objects to boxes (as in annotation) and increasing coverage. The background is not subject of the loss and is separate instance.

\begin{equation}
    \mathcal{L}_{shape} = \arg \max_{b_c} \sum_{i \in C^*} U(p_i,b) o_i^{C^*} -  \sum_{i \in P \setminus C} U(p_i, b)
\end{equation}

==> methods.tex <==
\section{Methods}

% scheme cycle, equation cycle, Scheme-architecture, pustit normals ablation na lidarech

\textbf{Point clouds and scene flow.}
% jak udelat z R matici? kombinuju dve notace dohromady
A point cloud is an unordered set of 3D points $\set{X}\subset\mathbb{R}^{3}$. 
Given a paired temporal sequence, a \emph{source point cloud}
consists of points $\mathbf{x}\in\set{X}$ measured at time $t$ and a \emph{target point cloud} consists of points $\mathbf{y}\in\set{Y}$
measured at time $t + dt$.
The scene flow is a 3D motion field
$\set{F} = \{\vect{f}_\vect{x}\;|\; \vect{f}_\vect{x} \in \mathbb{R}^{3}\}$, where $\vect{f}_\vect{x}$ denotes the motion of point $\vect{x}$ in time $dt$. %Points matching strategy and correspondences estimation is explained in the next subsection.

We approach the problem of scene flow estimation by adopting self-supervised architecture for flow regression and enhance it with our novel self-supervised losses. An illustration of our proposed loss functions is depicted in the bottom half of the Figure \ref{fig:overview}. 
% 
% \DHu{[potentially remove following sentence]} The state-of-the-art baseline and our contribution to it are described in the following paragraphs.

%We jointly supervise the flow regression via visibility-aware chamfer distance and \oursmooth with \surface. Our method first computes the initial free space representation and Euclidean neighborhoods for smoothness. Then, during each iteration of Chamfer distance, we use pre-computed warped flow neighbors to propagate the cyclic smoothness. 


\subsection{Self-supervised learning baseline}
If no annotations are available, a typical self-supervised loss attracts the flow applied on the source point cloud $\vect{x} + \vect{f}_\vect{x}$ towards the closest point in the target point cloud $\vect{y}$ via
the nearest-neighbor distance loss originally proposed in~\cite{Mittal_2020_CVPR}:
%
%The loss attracts the flow from point $\vect{x}_i + \mathbf{f}_i$, we find its target as the nearest neighbors from $\set{Y}$ using Euclidean distance:
%
\begin{equation}
    \mathcal{L}_{dist}(\set{F}) = \frac{1}{|\set{X}|} \sum_{\vect{x} \in \set{X}} \min_{\vect{y} \in \set{Y}} \| \vect{x} + \mathbf{f}_\vect{x} - \vect{y}\|^2_2 
    \label{eq:distance}
\end{equation}
%
By minimizing the distance loss, we bring the warped point cloud $\set{X} + \set{F}$ closer to the target $\set{Y}$. Since there is no assumption about the rigidity of objects in the scene, each point is allowed to flow independently; therefore, the resulting flow would deform objects substantially. To ensure that the flow field respects the rigidity of objects, authors estimate for each point $\vect{x}$ \emph{a rigid cluster} $R(\vect{x})$ - a set of points that are assumed to lie on a common rigid object. Typical implementation~\cite{FlowStep3D, lang2023scoop} considers just the set $N_X(\mathbf{x})$ of $k$-nearest neighbours of $\vect{x}$ from $X$.
%\begin{flalign}    
%&R(\vect{x}) = N_X(\mathbf{x})=\\
%    &\{\mathbf{r} \; | \; \|\vect{x}-\vect{r}\|_2\leq\|\vect{x}-\vect{r}^\prime\|_2, \vect{r}^\prime\not\in N_X(\mathbf{x}),\;  |N_X(\mathbf{x})|=k\} \nonumber,
%\end{flalign}
Once a definition of rigid cluster $R$ is available,  the smoothness of the flow $F$ is enforced through smoothness loss:
%\DHu{here $R(\vect{x}) = N_X(\mathbf{x})$. Later we work with the rigid cluster as if it is the neighborhood. Do we need $R(\vect{x})$ in the notation?}:
%
% \textbf{Smoothness regularization}
\begin{equation}
    \mathcal{L}_{sm}(F, R) = \frac{1}{|\set{X}|k_f} \sum_{\vect{x}_i \in \set{X}} \sum_{\vect{r} \in R(\vect{x})}\| \vect{f}_\vect{x} - \vect{f}_\vect{r}\|_1
    \label{eq:smootness}
\end{equation}
% 
It is desirable to have the rigid cluster as large as possible, however, the higher the number of considered neighbors $k$, the higher the risk of connecting multiple independent rigid objects into a common rigid cluster. Therefore, $k$ has to stay relatively small, which causes that rigid objects are disintegrated into small pieces, and the underlying smoothness loss is inefficient. 
%
Towards this end, we enhance the definition of the rigid cluster to respect spatio-temporal consistency of objects. In particular, we extend the definition by explicitly reconstructing the surface of objects, and consider cyclic consistency between the rigid clusters in the source and target point clouds.



% \DHu{[The following sentence is not very clear ...]} This over-segmentation can lead to matching of source points to the object's different parts in the target point cloud. We can enlarge the neighborhood by increasing the $k_f$ to group more source points, but then we risk the opposite problem of \textit{under-segmentation}. 


\subsection{Surface smoothness}\label{sec:L_surf}
%
We improve the definition of rigid cluster by introducing also the local surface similarity. Such idea can help in cases where objects are close to planar surface or where we need to separate two spatially close objects with different flows. 

We choose to approximate the problem by estimating the normal $\vect{n}_\vect{x}$ of the surface in point $\vect{x}$. 
\ifx\false
\DHu{[isn't this just regular surface normal? Why explaining it through the tangent?]}. \PV{there are more ways how to construct normal, It is just basic stuff, but I wanted to specify it. Another can be fitting something else than plane.}
%
The solution for estimating the surface normal is therefore reduced to a simple analysis of the eigenvectors and eigenvalues (PCA) of a covariance matrix created from the nearest neighbors of the query point $\vect{x}_i$. More specifically, for each point $\vect{x}_i$, we compute the covariance matrix $\mat{C}$ from its neighborhood points $\vect{x}_r \in \set{N}_X(\vect{x}_i)$ \DHu{[perhaps not necessary to have a standalone equation for cov. matrix.]} \PV{agree, it is more about indexing. We can leave it out and just describe it as well}:
%
\begin{equation}
    \mat{C} = \frac{1}{k_n} \sum_{i=0}^{k_n} (\vect{x}_i - \overline{\vect{x}}) (\vect{x}_i - \overline{\vect{x}})^\top, \overline{\vect{x}} = \frac{1}{k_n} \sum_{i=0}^{k_n} \vect{x}_r
\end{equation}
%
The surface normal $\vect{n}_i$ is computed as the eigenvector of \mat{C} corresponding to its smallest eigenvalue.
%
The $k_n$ denotes the number of nearest neighbors considered for normal estimation. % used in the approximation of the plane points.
%
\fi
We follow the method described in~\cite{Tombari10} for sign disambiguation, which is implemented in the open-source Pytorch3D library. The computed normal vector $\vect{n}_\vect{x}$ of point $\vect{x}$
forms surface-aware descriptor
$\phi_\vect{x} = [\vect{x}^T, \vect{n}_\vect{x}^T ]^T$ that allows to uncover more reliable \emph{surface-aware rigid cluster}
\begin{equation}
    R_{\textit{surf}}(\vect{x}) = N_\Phi(\phi_\vect{x}),
\end{equation}
where $N_\Phi : \mathbb{R}^{6} \rightarrow \{\mathbb{R}^{3}\}$ is again calculating the nearest neighborhood, but this time with six dimensional input while returning a set of 3D points. Surface-aware smoothness loss is then defined as follows:
%
\begin{equation}
    \mathcal{L}_{\textit{surf}}(F) = \mathcal{L}_{\textit{sm}}(F, R_{\textit{surf}})
    \label{eq:smootness-normals}
\end{equation}
%
%\DHu{[here $R_{\textit{surf}}$ is 6D and original $\mathcal{L}_{\textit{sm}}$ works with 3D $R$].}
By using the $\mathcal{L}_{surf}$ instead of regular smoothness from eq. (\ref{eq:smootness}), we weight correspondences on similarly-looking surfaces rather than only close pairs.
%\KZ{You should be consistent $\mathcal{L}_{\textit{surf}}$ vs $\mathcal{L}_{surf}$}

\subsection{Cyclic smoothness}\label{sec:L_csm}
In this section, we introduce \textit{cyclic smoothness rigid clusters} that propagate the information about object rigidity from the target point cloud back to source via matched correspondences, thus enforcing flow $\vect{f}_{\vect{x}}$ navigating to the matching surface parts, see Figure \ref{fig:cyclev2}. 
%
% \begin{figure*}[t]
%     \centering
%     \includegraphics[width=0.99\linewidth]{img/cyclic_smooth.png}
%     \caption{Cyclic smoothness, \todo{write indices to figure, when fixed}}
%     \label{fig:computation-of-ff}
% \end{figure*}
%
%
\begin{figure}[t]
    \centering
    \includegraphics[width=0.95\linewidth]%{img/cyclic_smooth_v2.png}
    {img/cyclic_smoothness.jpg}
    \caption{\textbf{Cyclic Smoothness loss}  $\mathcal{L}_{csm}$ enforces the same flow 
    % (\tikzcircle[fill={rgb:red,1.;green,2.;blue,0.2}]{3pt}) 
    (dashed green arrow)
    % \DHu{[istead of green dot we should have green dashed arrow]} 
    over the  rigid cluster $R_c(\vect{x})$ (light blue set). The $R_c(\vect{x})$ is constructed as follows: Given the source point \vect{x} (\tikzcircle[fill={rgb:red,0.1;green,1.9;blue,3.17}]{3pt}), we find its nearest neighbor \vect{y_x^*} in target point cloud  (\tikzcircle[fill={rgb:red,3.5;green,0.2;blue,0.}]{3pt}). Then we estimate the rigid neighborhood $N_Y(\vect{y_x^*})$ (light red set) of $\vect{y_x^*}$ . Finally, any source point $\vect{r}$ whose flow $\vect{r}+\vect{f}_\vect{r}$ has the nearest neighbour in $N_Y(\vect{y_x^*})$ is added to the rigid cluster $R_c(\vect{x})$.
    % 
    %to gather points from source, which warped flows (\tikzcircle[fill={rgb:red,1.;green,2.;blue,0.2}]{3pt}) match within the points of the same neighborhood $N_Y(\vect{y_x^*})$, i.e. the $\vect{r}$. Lastly, we apply $\mathcal{L}_{csm}$ to the corresponding points in cycle, the $\vect{x}$ and $\vect{r}$. The points are not in each others neighborhoods in source point cloud, therefore the regular smoothness loss would not prevent the degenerative solution.
    % \DHu{notation adaptation needed wrt re-written Method section} \KZ{Should not we replace NN by $\mathcal{L}_{dist}$?}\PV{Here it should denote nearest neigbor, because it is a tool not only for $\mathcal{L}_{dist}$, but for cyclic smoothness as well, also add the smooth neighborhood}
    }
    \label{fig:cyclev2}
\end{figure}


% First, we compute the Euclidean neighborhood \DHu{$\ell$} in target point cloud $\ell=N_Y(\vect{y}_r)$ of size $k_f$, to find points that belong to the same rigid object as in (\ref{eq:smootness}) \DHu{$\ell$ here is different than $\ell$ in equation 5 - needs correction}. Then
First, we leverage the pre-computed neighborhood $N_X(\vect{x})$ from the distance term (\ref{eq:distance}) and denote the nearest point from $Y$ to $\vect{x}+\vect{f}_{\vect{x}}$ as $$\vect{y}^\star_{\vect{x}}=\arg\min_{\vect{y}\in Y}\|\mathbf{x}+\vect{f}_{\vect{x}}-\mathbf{y} \|_2^2.$$
Then we define the \textit{cyclic smoothness rigid cluster} of point $\vect{x}$ as a set of points $\vect{r}\in X$ such that their flow falls within the neighbourhood of $\vect{y}^\star_\vect{x}$. More formally:
\begin{equation}
    R_c(\vect{x})=\{\vect{r}\; | \; \vect{r}+\vect{f}_\vect{r} \in  N_Y(\vect{y}^\star_\vect{x})\}
\end{equation}
The cycle-consistent smoothness loss is then defined as follows:
%   
% After calculation of indices, we apply smoothness to the source points:
%
% 
\begin{equation}
    \mathcal{L}_{csm}(F) = \mathcal{L}_{sm}(F, R_c)
    \label{eq:cycle-smootness}
\end{equation}
%
Note that we do not introduce any extra parameter when constructing the cyclic smoothnes compared to regular smoothness loss. 
% \KZ{I do not know what is meant by that} \PV{We do not need extra tunning or introduction of parameters compared to smoothness loss implementation (number of NN for example)}


% \subsection{Visibility-aware scene flow}
% % drop visibility-aware smoothness
% % paragraph that says points data representation omits the important features of how it was acquired?

% We introduce a free space loss as a new regularization term for pushing out the flow from unoccupied spots observable through the visibility of target point cloud $Y$. By defining $\mathcal{F}_y \in \mathcal{R}^3$ as a see-through area in the target time, we know that none of the flows can end up inside, otherwise they would naturally occlude the measurement of $Y$, see Figure \ref{fig:freespace}. Such regularization prevents the optimization from being stuck in local minima, where smoothness prevents the distance loss from converging inside the free space area. We define a binary free space label $o_i$ for each point $\vect{x}_i \in \set{X}$ as an indication of flow in an unoccupied area:
% %
% \begin{figure}[t]
%     \centering
%     \includegraphics[width=0.9\linewidth]{img/overview-visibility_v1.png}
%     \caption{Freespace area}
%     \label{fig:freespace}
% \end{figure}
% %
% \begin{equation}
%     o_i= 
%     \begin{cases}
%     1, & \text{if} ~ \vect{x}_i + \vect{f}_i \in \mathcal{F}_y \\
%     0,              & \text{otherwise}
%     \end{cases}
% \end{equation}
% %
% Then we use the masked points to compute the free-space loss $\mathcal{L}_\mathcal{F}$ to repel warped points with the flow ($\hat{\vect{x}}_i$) outside of the $\mathcal{F}_y$ towards its boundary represented by $y_i \in Y$. We leverage pre-computed nearest neighbors from distance loss and define the free-space loss term as follows:
% % boundary define as N_Y
% \begin{equation}
%     \mathcal{L}_{\mathcal{F}} = \frac{1}{|\set{X}|} \sum_{\vect{x}_i \in \set{X}} o_i \min_{\vect{y}_j \in \set{Y}} \| \hat{\vect{x}}_{i} - \vect{y}_j \| ^2_2 
% \end{equation}
% %
% %

% \subsection{Efficient implementation of freespace}
% % vykostit rovnici a citovat
% A naive implementation of $\mathcal{F}_y$ in 3D space is technically intractable and inefficient. Therefore we implement $\mathcal{F}_y$ as a 2D range image representing the frontal view of the point cloud $\set{Y}$. We use spherical projection as in \cite{chen2021icra} to create  range image $D_Y$, where each pixel contains the nearest 3D point, which is converted to spherical coordinates and further to image coordinates $u,v$, see Figure \ref{fig:freespace}.
% % \begin{equation}
% %     \begin{pmatrix}
% %         u \\ v 
% %     \end{pmatrix}
% %         =
% %     \begin{pmatrix}
% %             \frac{1}{2}[1 - \arctan(p_y,p_x).\pi^{-1}]w \\
% %             [1 - (\arcsin(p_zd^{-1}) + fov_{up})fov^{-1}]h
% %     \end{pmatrix}
% % \end{equation}
% % %
% % where $d = \|p\|_2$ is the range, $fov=fov_{up} + fov_{down}$ is the vertical field of view of the sensor. Given the image coordinates $u$, $v$ and range $d$, we generate the range image $D_Y$ from the target point cloud, .

% Next, we compute the depth image coordinates of the warped point cloud $X+F$ during each iteration of training and compare its per-point depth $d_i$ with the depth corresponding $u_i$ and $v_i$ coordinates in the $D_Y$ to find the free space label:
% %
% \begin{equation}
%     o_i= 
%     \begin{cases}
%     1, & \text{if} ~ d_i < D_Y(u_i, v_i) \\
%     0,              & \text{otherwise}
%     \end{cases}
% \end{equation}
% %
% where the indication label $o_i$ represents points in free space, i.e. the flow, that occludes the target points $y_i$ in frontal view.
% %
% % Here I need to set up the equations


 

% \begin{figure}[h]
%     \centering
%     \includegraphics[width=0.9\linewidth]{img/visibility-efficient implementation.png}
%     \caption{Computation of freespace}
%     \label{fig:vis-efficient-implementation}
% \end{figure}
% we guide / enchance chamfer distance by constrained visible area called freespace

% \begin{figure}[h]
%     \centering
%     \includegraphics[width=0.9\linewidth]{img/visibility_mechanism_2d.png}
%     \caption{Visibility mechanism. Include the cost function as heatmap from lidar origin}
%     \label{fig:visibility-mechanism}
% \end{figure}



\subsection{Training objective and Architecture}
% 
% \PV{TODO:CHECK}
We build upon the existing scene flow neural architectures, namely SCOOP~\cite{lang2023scoop} for bijective mappings in stereo datasets and Neural Prior~\cite{li2021neural} for real LiDARs, and produce the flow field $F$ from the inputs with the neural network. We directly backpropagate through the flows to the weights of the network to minimize our proposed loss terms. That way, our proposed losses can be used for arbitrary architecture, see Figure \ref{fig:architercture2}.
% We jointly train the network to minimize proposed loss functions. 
The final training objective is:
%
\begin{equation}
    \mathcal{L} = \mathcal{L}_{dist} + \alpha_{surf} \mathcal{L}_{surf} + \alpha_{csm} \mathcal{L}_{csm}
\end{equation}
%
where $\alpha_{surf}$ and $\alpha_{csm}$ are hyperparameters balancing the contribution of individual loss terms. 
% Note that we keep the $\mathcal{L}_{sm}$ for rigid clusters smoothness in source neighborhoods as they are not part of the $\mathcal{L}_{csm}$.

%%%% VERSION 1
% \section{Methods}

% % scheme cycle, equation cycle, Scheme-architecture, pustit normals ablation na lidarech

% \textbf{Point clouds and scene flow.}
% % jak udelat z R matici? kombinuju dve notace dohromady
% A point cloud is an unordered set of 3D points. 
% Given a paired temporal sequence, a source point cloud
% $\set{X}=\{\vect{x}_i \in R^{3}\}$ at frame $t$ and target point cloud
% $\set{Y}= \{\vect{y}_j \in R^{3}\}$ at frame $t + 1$,
% the scene flow estimates the 3D motion field
% $\set{F} = \{\vect{f}_i \in R^{3}\}$ for frame $t$ with $f_i$ denoting a 3D motion vector in between the corresponding points from source and target point clouds. Points matching strategy and correspondences estimation is explained in the next subsection.

% We approach the problem of scene flow estimation by adopting self-supervised architecture for flow regression~\cite{li2021neural, lang2023scoop} and enhance it with our novel self-supervised loss terms during the optimization/learning without the need for ground truth labels. An illustration of our loss functions is depicted in \PV{[come back after refining the figure]} the lower part of Figure \ref{fig:overview}. We jointly \DHu{\st{optimize} supervise]} the flow regression via visibility-aware chamfer distance and \oursmooth with \surface. Our method first computes the initial free space representation and Euclidean neighborhoods for smoothness. Then, during each iteration of Chamfer distance, we use pre-computed warped flow neighbors to propagate the cyclic smoothness. 


% \subsection{Matching the correspondences}
% In order to establish point correspondences between the source $\set{X}$ and target $\set{Y}$ point clouds via estimated flow field $\set{F}$, we utilize the nearest-neighbor distance loss for warped point cloud $\hat{\vect{x}}_i=\vect{x}_i + \vect{f}_i$, as proposed in~\cite{Mittal_2020_CVPR}.
% %
% For each transformed point $\hat{\vect{x}}_i \in \widehat{\set{X}} = \set{X}+\set{F}$, we find its nearest neighbor $\vect{y}_j \in \set{Y}$ using Euclidean distance:
% %
% \begin{equation}
%     \mathcal{L}_{dist} = \frac{1}{|\set{X}|} \sum_{\hat{\vect{x}}_i \in \hat{\set{X}}} \min_{\vect{y}_j \in \set{Y}} \| \hat{\vect{x}}_{i} - \vect{y}_j \|^2_2 
%     \label{eq:distance}
% \end{equation}
% %
% By minimizing the distance loss, we bring the warped point cloud $\hat{\set{X}}$ closer to the target, but the coherence of geometric structures in time would not be preserved. To ensure that the flow field respects the rigid objects shapes we enforce the flow smoothness $\mathcal{L}_{sm}$ on neighboring source points similarly to~\cite{FlowStep3D, lang2023scoop}:
% %
% % \textbf{Smoothness regularization}
% \begin{equation}
%     \mathcal{L}_{sm} = \frac{1}{|\set{X}|k_f} \sum_{\vect{x}_i \in \set{X}} \sum_{\ell \in N_X(\vect{x}_i)}\| \vect{f}_i - \vect{f}_\ell\|_1
%     \label{eq:smootness}
% \end{equation}
% % 
% where $N_X(\vect{x}_i)$ is an Euclidean neighborhood of $\vect{x}_i$ in $\set{X}$ of size $k_f$, where $k_f$ is the number of neighboring points. 
% %
% However, the smoothness neighborhood tends to disintegrate objects into small rigid clusters with a consistent flow, but not consistent in the full body of the object.
% %
% We can enlarge the neighborhood by increasing the $k_f$, but then we risk connection of two close object inside one neighboorhood.

% % \DHu{[The following sentence is not very clear ...]} This over-segmentation can lead to matching of source points to the object's different parts in the target point cloud. We can enlarge the neighborhood by increasing the $k_f$ to group more source points, but then we risk the opposite problem of \textit{under-segmentation}. 


% \subsection{Surface smoothness}
% %
% We further improve the smoothness by grouping the points with respect to the local surface of point cloud. Such idea can help in cases where objects are close to planar background or where we need to separate two close objects with different flows. 

% We choose to approximate the problem by estimation of the normal of a plane tangent to the surface \DHu{[isn't this just regular surface normal? Why explaining it through the tangent?]}. \PV{there are more ways how to construct normal, It is just basic stuff, but I wanted to specify it. Another can be fitting something else than plane.}
% %
% The solution for estimating the surface normal is therefore reduced to a simple analysis of the eigenvectors and eigenvalues (PCA) of a covariance matrix created from the nearest neighbors of the query point $\vect{x}_i$. More specifically, for each point $\vect{x}_i$, we compute the covariance matrix $\mat{C}$ from its neighborhood points $\vect{x}_r \in \set{N}_X(\vect{x}_i)$ \DHu{[perhaps not necessary to have a standalone equation for cov. matrix.]} \PV{agree, it is more about indexing. We can leave it out and just describe it as well}:
% %
% \begin{equation}
%     \mat{C} = \frac{1}{k_n} \sum_{i=0}^{k_n} (\vect{x}_i - \overline{\vect{x}}) (\vect{x}_i - \overline{\vect{x}})^\top, \overline{\vect{x}} = \frac{1}{k_n} \sum_{i=0}^{k_n} \vect{x}_r
% \end{equation}
% %
% The surface normal $\vect{n}_i$ is computed as the eigenvector of \mat{C} corresponding to its smallest eigenvalue.
% %
% The $k_n$ denotes the number of nearest neighbors considered for normal estimation. % used in the approximation of the plane points.
% %
% We follow the method in~\cite{Tombari10} for sign disambiguation, which is implemented in the open-source Pytorch3D library. The computed normal vector $\vect{n}_i$ is then concatenated with geometrical features of $\vect{x}_i$ to assemble neighborhood $N_n$ respectively for \DHu{surface} smoothness calculation \DHu{[I almost missed the tiny difference of surf loss and smoothness loss ... maybe different notation would help to enhance the difference]}\PV{Well, the prescription is almost the same, the difference is how to get the indices, I will look at it}:
% % Zadefinovat specialni neighborhood N_n pro normaly
% %
% \begin{equation}
%     \mathcal{L}_{\textit{surf}} = \frac{1}{|\set{X}|k_f} \sum_{\vect{x}_i \in \set{X}} \sum_{\ell \in N_X([\vect{x}_i, \vect{n}_i])}\| \vect{f}_i - \vect{f}_\ell\|_1
%     \label{eq:smootness-normals}
% \end{equation}
% %
% By using the $\mathcal{L}_{surf}$ instead of regular smoothness from eq. (\ref{eq:smootness}), we weight correspondences on similar-looking surfaces rather than only close pairs.

% \subsection{Cyclic smoothness}
% To further mitigate the problem of noisy source points grouping, we introduce \textit{cyclic smoothness} to augment the loss with smoothness propagation from target points back to source points via matched correspondences, thus enforcing flows navigating the to same object parts to be consistent, see Figure \ref{fig:cyclev2}.
% %
% % \begin{figure*}[t]
% %     \centering
% %     \includegraphics[width=0.99\linewidth]{img/cyclic_smooth.png}
% %     \caption{Cyclic smoothness, \todo{write indices to figure, when fixed}}
% %     \label{fig:computation-of-ff}
% % \end{figure*}
% %
% %
% \begin{figure}[t]
%     \centering
%     \includegraphics[width=0.95\linewidth]{img/cyclic_smooth_v2.png}
%     \caption{Cyclic Smoothness loss $\mathcal{L}_{csm}$.
%     \tikzcircle[fill={rgb:red,0;green,1;blue,1.5}]{3pt},
%     \tikzcircle[fill={rgb:red,1.5;green,0;blue,0.5}]{3pt},
%     \tikzcircle[fill={rgb:red,0;green,1.5;blue,0.5}]{3pt}.
%     }
%     \label{fig:cyclev2}
% \end{figure}


% % First, we compute the Euclidean neighborhood \DHu{$\ell$} in target point cloud $\ell=N_Y(\vect{y}_r)$ of size $k_f$, to find points that belong to the same rigid object as in (\ref{eq:smootness}) \DHu{$\ell$ here is different than $\ell$ in equation 5 - needs correction}. Then
% First, we leverage the pre-computed neighborhood from the distance term (\ref{eq:distance}) and denote the nearest point $\vect{y}_r$ of warped point $\vect{\hat{x}_i}$ as:
% %
% \begin{equation}
%     \vect{y}_r= \underset{\vect{y}_j \in \set{Y}}{\mathrm{argmin}} \|(\hat{\vect{x}}_i - \vect{y}_j \|^2_2    
% \end{equation}
% %
% Then we gather indices  corresponding to the neighborhood of $\vect{y}_r$, denoted $L = N_Y(\vect{y_r})$, from the target point cloud and finally propagate the joint indices to the source point cloud as $J(i) = \{j, l\}$, where $J(i)$ denotes the set of indices in $X$, that we will smooth according to the following: \PVc{I am still not sure with the exact notation, I read about index sets, but not used to it in this setup, but the scheme is consistent. Karel or David pls verify.}
% %   
% % After calculation of indices, we apply smoothness to the source points:
% %
% % 
% \begin{equation}
%     \mathcal{L}_{csm} = \frac{1}{|\set{X}|} \sum_{\vect{x}_i \in \set{X}} \sum_{l \in \set{L}} \|\vect{f}_i - \vect{f}_l \|_1
%     \label{eq:cycle-smootness}
% \end{equation}
% %
% Note that no extra parametrization compared to smoothness loss is needed.


% \subsection{Visibility-aware scene flow}
% % drop visibility-aware smoothness
% % paragraph that says points data representation omits the important features of how it was acquired?

% We introduce a free space loss as a new regularization term for pushing out the flow from unoccupied spots observable through the visibility of target point cloud $Y$. By defining $\mathcal{F}_y \in \mathcal{R}^3$ as a see-through area in the target time, we know that none of the flows can end up inside, otherwise they would naturally occlude the measurement of $Y$, see Figure \ref{fig:freespace}. Such regularization prevents the optimization from being stuck in local minima, where smoothness prevents the distance loss from converging inside the free space area. We define a binary free space label $o_i$ for each point $\vect{x}_i \in \set{X}$ as an indication of flow in an unoccupied area:
% %
% \begin{figure}[t]
%     \centering
%     \includegraphics[width=0.9\linewidth]{img/overview-visibility_v1.png}
%     \caption{Freespace area}
%     \label{fig:freespace}
% \end{figure}
% %
% \begin{equation}
%     o_i= 
%     \begin{cases}
%     1, & \text{if} ~ \vect{x}_i + \vect{f}_i \in \mathcal{F}_y \\
%     0,              & \text{otherwise}
%     \end{cases}
% \end{equation}
% %
% Then we use the masked points to compute the free-space loss $\mathcal{L}_\mathcal{F}$ to repel warped points with the flow ($\hat{\vect{x}}_i$) outside of the $\mathcal{F}_y$ towards its boundary represented by $y_i \in Y$. We leverage pre-computed nearest neighbors from distance loss and define the free-space loss term as follows:
% % boundary define as N_Y
% \begin{equation}
%     \mathcal{L}_{\mathcal{F}} = \frac{1}{|\set{X}|} \sum_{\vect{x}_i \in \set{X}} o_i \min_{\vect{y}_j \in \set{Y}} \| \hat{\vect{x}}_{i} - \vect{y}_j \| ^2_2 
% \end{equation}
% %
% %

% \subsection{Efficient implementation of freespace}
% % vykostit rovnici a citovat
% A naive implementation of $\mathcal{F}_y$ in 3D space is technically intractable and inefficient. Therefore we implement $\mathcal{F}_y$ as a 2D range image representing the frontal view of the point cloud $\set{Y}$. We use spherical projection as in \cite{chen2021icra} to create  range image $D_Y$, where each pixel contains the nearest 3D point, which is converted to spherical coordinates and further to image coordinates $u,v$, see Figure \ref{fig:freespace}.
% % \begin{equation}
% %     \begin{pmatrix}
% %         u \\ v 
% %     \end{pmatrix}
% %         =
% %     \begin{pmatrix}
% %             \frac{1}{2}[1 - \arctan(p_y,p_x).\pi^{-1}]w \\
% %             [1 - (\arcsin(p_zd^{-1}) + fov_{up})fov^{-1}]h
% %     \end{pmatrix}
% % \end{equation}
% % %
% % where $d = \|p\|_2$ is the range, $fov=fov_{up} + fov_{down}$ is the vertical field of view of the sensor. Given the image coordinates $u$, $v$ and range $d$, we generate the range image $D_Y$ from the target point cloud, .

% Next, we compute the depth image coordinates of the warped point cloud $X+F$ during each iteration of training and compare its per-point depth $d_i$ with the depth corresponding $u_i$ and $v_i$ coordinates in the $D_Y$ to find the free space label:
% %
% \begin{equation}
%     o_i= 
%     \begin{cases}
%     1, & \text{if} ~ d_i < D_Y(u_i, v_i) \\
%     0,              & \text{otherwise}
%     \end{cases}
% \end{equation}
% %
% where the indication label $o_i$ represents points in free space, i.e. the flow, that occludes the target points $y_i$ in frontal view.
% %
% % Here I need to set up the equations


 

% \begin{figure}[h]
%     \centering
%     \includegraphics[width=0.9\linewidth]{img/visibility-efficient implementation.png}
%     \caption{Computation of freespace}
%     \label{fig:vis-efficient-implementation}
% \end{figure}
% we guide / enchance chamfer distance by constrained visible area called freespace

% % \begin{figure}[h]
% %     \centering
% %     \includegraphics[width=0.9\linewidth]{img/visibility_mechanism_2d.png}
% %     \caption{Visibility mechanism. Include the cost function as heatmap from lidar origin}
% %     \label{fig:visibility-mechanism}
% % \end{figure}



% \subsection{Network for flow regression}
% % Production of flow from source and target point clouds
% % already regularizations
% % refinements
% % Networks for flow
% % implementation
% \PV{working on this section, note yet completed}
% We choose to apply our loss functions on top of the two top-performing architectures, SCOOP~\cite{lang2023scoop} that is the current state-of-the-art method on stereoKITTI dataset, and Neural Prior~\cite{li2021neural} that is the current state-of-the-art on LiDAR scene flow datasets.
% %
% We directly backpropagate through the outputs from the networks to minimize our proposed loss terms. Our full framework is depicted on Figure \ref{fig:architecture}.
% % 
% \begin{figure*}
%     \centering
%     \includegraphics[width=0.99\linewidth]{img/overview-Architecture.png}
%     \caption{Model exchangeable, enhanced rigidity block ours, left-side represent the baseline, our contribution marked in red, note current target is next source, black arrows are nearest neighboors, arrows from Nx should split but start same. Encapsulate smoothness with surface-aware smoothness. }
%     \label{fig:architecture}
% \end{figure*}

% % scheme
% % description of SCOOP/Prior?

% % \begin{figure*}[h]
% %     \centering
% %     \includegraphics[width=0.9\linewidth]{img/visibility-aware-smootness.png}
% %     \caption{Visibility to cut KNN connections.}
% %     \label{fig:visibility-smoothness}
% % \end{figure*}

% % \subsection{Training objective}

% \subsection{Training loss term}
% Lastly, we jointly train the flow to minimize proposed loss functions. The final training objective is:
% %
% \begin{equation}
%     \mathcal{L} = \mathcal{L}_{dist} + \alpha_{sm} \mathcal{L}_{sm} + \alpha_{csm} \mathcal{L}_{csm}
% \end{equation}
% %
% where $\alpha_{surf}$ and $\alpha_{csm}$ are hyperparameters balancing the contribution of individual loss terms.
